Homeomorphism Prior for False Positive and Negative Problem in Medical Image Dense Contrastive Representation Learning

Dense contrastive representation learning (DCRL) has greatly improved the learning efficiency for image-dense prediction tasks, showing its great potential to reduce the large costs of medical image collection and dense annotation. However, the properties of medical images make unreliable correspondence discovery, bringing an open problem of large-scale false positive and negative (FP&N) pairs in DCRL. In this paper, we propose GEoMetric vIsual deNse sImilarity (GEMINI) learning which embeds the homeomorphism prior to DCRL and enables a reliable correspondence discovery for effective dense contrast. We propose a deformable homeomorphism learning (DHL) which models the homeomorphism of medical images and learns to estimate a deformable mapping to predict the pixels' correspondence under topological preservation. It effectively reduces the searching space of pairing and drives an implicit and soft learning of negative pairs via a gradient. We also propose a geometric semantic similarity (GSS) which extracts semantic information in features to measure the alignment degree for the correspondence learning. It will promote the learning efficiency and performance of deformation, constructing positive pairs reliably. We implement two practical variants on two typical representation learning tasks in our experiments. Our promising results on seven datasets which outperform the existing methods show our great superiority. We will release our code on a companion link: https://github.com/YutingHe-list/GEMINI.

==> tex/Acknowledgments.tex <==
\section*{Acknowledgments}
This research was supported by the National Key Research and Development Program of China (No. 2021ZD0113202), National Natural Science Foundation under grants (61828101, 62101249), Natural Science Foundation of Jiangsu Province (BK20210291), Excellence Project Funds of Southeast University, CAAI-Huawei MindSpore Open Fund, and Scientific Research Foundation of Graduate School of Southeast University (YBPY2139). We thank the Big Data Computing Center of Southeast University for providing the facility support on the numerical calculations. 

==> tex/bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yutinghe}}]{Yuting He} is now a research associate in Case Western Reverse University. He received B.E. degree in Hefei University of Technology, Hefei, China in 2018, and the Ph.D. degree from the Southeast University, Nanjing, China in 2023. He also visited Western University, London, Canada in 2022. His research focuses on developing novel methodologies to learn more efficient extraction of knowledge in medical information for computer-aided diagnosis, surgery and medical imaging.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/boyuwang}}]{Boyu Wang} (Member, IEEE) received the BEng degree in electronic information engineering from Tianjin University, Tianjin, China, the MSc degree in electrical and computer engineering from the University of Macau, Macau, China, and the PhD degree in computer science from McGill University, Montreal, QC, Canada. He is currently an assistant professor with the Department of Computer Science, University of Western Ontario, London, ON, Canada, where he is also affiliated with Western Centre for Brain and Mind and the Vector Institute. He was a post-doctoral research fellow with the University of Pennsylvania, Philadelphia, PA, USA, and Princeton University, Princeton, NJ, USA. His research interests include machine learning theory, algorithms, and applications. He has authored or co-authored more than 60 research papers in top venues, including ICML, NeurIPS, ICLR, CVPR, AAAI, IJCAI, AISTATS, Journal of Machine Learning Research, IEEE Transactions on Pattern Analysis and Machine Intelligence, etc.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/rongjunge}}]{Rongjun Ge} received the B.E. and M.E. degrees from the School of Information Science and Engineering, Lanzhou University, Lanzhou, China, in 2013 and 2016, and the Ph.D. degree from the Laboratory of Image Science and Technology, School of Computer Science and Engineering, Southeast University, Nanjing, China. He is currently a assistant professor with the College of Computer Science and Technology, Nanjing University of Aeronautics and Astronautics, Nanjing, China. His current research interests include medical image processing and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/yangchen}}]{Yang Chen} received the M.S. and Ph.D. degrees in biomedical engineering from First Military Medical University, China, in 2004 and 2007, respectively. Since 2008, he has been a Faculty Member with the Department of Computer Science and Engineering, Southeast University, China. His recent work concentrates on the medical image reconstruction, image analysis, pattern recognition, and computerized-aid diagnosis.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/guanyuyang}}]{Guanyu Yang} received the B.S. degree and M.S. degree in biomedical engineering from Southeast University, Nanjing, China in 2002 and 2005 respectively, and joint Ph.D. degree with the Laboratory of Image Science and Technology, Southeast University, and Laboratoire Traitement du signal et de l’Image, University of Rennes 1, in 2011. He is a professor in the School of Computer Science and Engineering in Southeast University, Nanjing, China. His research interests are focused on deep learning in medical imaging, computer-assisted systems for diagnosis and therapy in medicine.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio/shuoli}}]{Shuo Li} is a global leader in conducting multi-disciplinary research to enable artificial intelligence (AI) in healthcare. He is a chair professor at Case Western Reserve University. Before that, he was an associate professor in the Western University and a scientist at the Lawson Health Research Institute. He was a scientist at GE Healthcare (2006-2015). He is a committee member in multiple highly influential conferences and societies. He is most notable for serving on the prestigious board of directors in the MICCAI society (2015-2024), where he is also the general chair for the MICCAI 2022 conference, which is the most influential AI-in-imaging conference. He has over 300 publications, acted as the editor for six Springer books, and serves as an associate editor for several prestigious journals in the field. Throughout his career, he has received several awards from GE, various institutes, and international organizations. He is a Fellow of SPIE, AAIA, and AIMBE.
\end{IEEEbiography} 
